Alchemy: A benchmark and analysis toolkit for meta-reinforcement learning agents

There has been rapidly growing interest in meta-learning as a method for increasing the flexibility and sample efficiency of reinforcement learning. One problem in this area of research, however, has been a scarcity of adequate benchmark tasks. In general, the structure underlying past benchmarks has either been too simple to be inherently interesting, or too ill-defined to support principled analysis. In the present work, we introduce a new benchmark for meta-RL research, emphasizing transparency and potential for in-depth analysis as well as structural richness. Alchemy is a 3D video game, implemented in Unity, which involves a latent causal structure that is resampled procedurally from episode to episode, affording structure learning, online inference, hypothesis testing and action sequencing based on abstract domain knowledge. We evaluate a pair of powerful RL agents on Alchemy and present an in-depth analysis of one of these agents. Results clearly indicate a frank and specific failure of meta-learning, providing validation for Alchemy as a challenging benchmark for meta-RL. Concurrent with this report, we are releasing Alchemy as public resource, together with a suite of analysis tools and sample agent trajectories.

==> Alchemy NeurIPS final/preamble.tex <==
% # FONTS
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{lineno}
\usepackage{csquotes}
\usepackage{microtype}

% # LAYOUT
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xspace}
\usepackage{placeins}
\usepackage{wrapfig}


% # COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}
\colorlet{DarkBlue}{black!50!blue!100}
\colorlet{DarkRed}{black!15!red!100}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!40}{#1}}

% # FIGURES
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{pgf}

\graphicspath{{img/}}

\usetikzlibrary{bayesnet}
\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\definecolor{hexcolor0xbfbfbf}{rgb}{0.749,0.749,0.749}

\usetikzlibrary{arrows,automata,backgrounds}
\tikzset{>=latex}
\tikzstyle{none}   = [inner sep=0pt]
\tikzstyle{line}   = [ -, thick, shorten <=1pt, shorten >=1pt ]
\tikzstyle{arrow}  = [ ->, thick, shorten <=1pt, shorten >=1pt ]
\tikzstyle{ardash} = [ dashed, ->, thick, shorten <=1pt, shorten >=1pt ]

\tikzstyle{empty}=[circle,opacity=0.0,text opacity=1.0,inner sep=0pt]
\tikzstyle{box}=[rectangle,fill=White,draw=Black]
\tikzstyle{filled}=[circle,thick,fill=hexcolor0xbfbfbf,draw=Black]
\tikzstyle{hollow}=[circle,thick,fill=White,draw=Black]
\tikzstyle{param}=[rectangle,fill=Black,draw=Black,inner sep=0pt,minimum width=4pt,minimum height=4pt]
\tikzstyle{paramhollow}=[rectangle,thick,fill=White,draw=Black,inner sep=0pt,minimum
width=4pt,minimum height=4pt]

% # TABLES
\usepackage{booktabs, array}

% # BIBLIOGRAPHY AND LINKS
%\usepackage{natbib}
\usepackage[
  linktoc=all,
  pdfcenterwindow=true,
  bookmarks=true,
  colorlinks,
  citecolor=DarkBlue,
  linkcolor=DarkRed,
  urlcolor=DarkBlue]{hyperref}

\usepackage[all]{hypcap}

% # ALGORITHMS
\usepackage{listings}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\small}

% # MATHEMATICS
\usepackage{setspace}
\usepackage[cmex10]{amsmath}
\usepackage{mathtools,amssymb,amsthm}
\usepackage{bbm}
\usepackage{nicefrac}
\begingroup
\makeatletter
  \@for\theoremstyle:=definition,remark,plain\do{
    \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{
      \addtolength\thm@preskip\parskip
    }
  }
\endgroup

% # DEFINITION ENVS
\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem{cond}{Condition}%[section]
\newtheorem*{crit}{Criterion}
\newtheorem{ass}{Assumption}%[section]

% # PLAIN ENVS
\theoremstyle{plain}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{lem}{Lemma}%[section]
\newtheorem{cor}{Corollary}%[thm]

% # REMARK ENVS
\theoremstyle{remark}
\newtheorem*{exmp}{Example}
\newtheorem*{rem}{Remark}

% # MODIFICATIONS
\renewcommand{\qedsymbol}{$\blacksquare$}

% # PROBABILITY
\DeclareMathOperator{\g}{\,|\,}
\DeclareMathOperator{\gl}{\,\|\,}
\DeclareRobustCommand{\KL}[2]{\ensuremath{\operatorname{KL}\left(#1\;\|\;#2\right)}}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

% # DISTRIBUTIONS
\DeclareMathOperator{\Gam}{\operatorname{Gam}}
\DeclareMathOperator{\InvGam}{\operatorname{InvGam}}
\DeclareRobustCommand{\E}[1]{\ensuremath{\mathbb{E}\!\left[#1\right]}}
\DeclareRobustCommand{\Ed}[2]{\ensuremath{\mathbb{E}_{#1}\!\left[#2\right]}}
\DeclareRobustCommand{\Vd}[2]{\ensuremath{\mathbb{V}_{#1}\!\left[#2\right]}}
\DeclareRobustCommand{\Md}[2]{\ensuremath{\mathbb{M}_{#1}\!\left[#2\right]}}

% # MISCELLANEOUS
\DeclareRobustCommand{\sg}[1]{\ensuremath{\operatorname{sg}\left[#1\right]}}
\DeclareRobustCommand{\cat}[2]{\ensuremath{\left[#1 \,; #2 \right]}}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2} % < , >
\DeclareMathOperator*{\argmin}{arg\,min  \ }
\DeclareMathOperator*{\argmax}{arg\,max  \ }


% # ROMAN MATHEMATICS
\DeclareMathOperator{\rE}{{\mathbb{E}}}
\DeclareMathOperator{\rV}{{\mathbb{V}}}
\DeclareMathOperator{\rR}{{\mathbb{R}}}
\DeclareMathOperator{\rN}{{\mathbb{N}}}

% # CALIGRAPHIC MATHEMATICS
\DeclareMathOperator{\cA}{\mathcal{A}}
\DeclareMathOperator{\cB}{\mathcal{B}}
\DeclareMathOperator{\cC}{\mathcal{C}}
\DeclareMathOperator{\cD}{\mathcal{D}}
\DeclareMathOperator{\cE}{\mathcal{E}}
\DeclareMathOperator{\cF}{\mathcal{F}}
\DeclareMathOperator{\cG}{\mathcal{G}}
\DeclareMathOperator{\cH}{\mathcal{H}}
\DeclareMathOperator{\cI}{\mathcal{I}}
\DeclareMathOperator{\cJ}{\mathcal{J}}
\DeclareMathOperator{\cK}{\mathcal{K}}
\DeclareMathOperator{\cL}{\mathcal{L}}
\DeclareMathOperator{\cM}{\mathcal{M}}
\DeclareMathOperator{\cN}{\mathcal{N}}
\DeclareMathOperator{\cO}{\mathcal{O}}
\DeclareMathOperator{\cP}{\mathcal{P}}
\DeclareMathOperator{\cQ}{\mathcal{Q}}
\DeclareMathOperator{\cR}{\mathcal{R}}
\DeclareMathOperator{\cS}{\mathcal{S}}
\DeclareMathOperator{\cT}{\mathcal{T}}
\DeclareMathOperator{\cU}{\mathcal{U}}
\DeclareMathOperator{\cV}{\mathcal{V}}
\DeclareMathOperator{\cW}{\mathcal{W}}
\DeclareMathOperator{\cX}{\mathcal{X}}
\DeclareMathOperator{\cY}{\mathcal{Y}}
\DeclareMathOperator{\cZ}{\mathcal{Z}}

% # BOLD MATHEMATICS
\DeclareMathOperator{\ba}{\mathbf{a}}
\DeclareMathOperator{\bb}{\mathbf{b}}
\DeclareMathOperator{\bc}{\mathbf{c}}
\DeclareMathOperator{\bd}{\mathbf{d}}
\DeclareMathOperator{\be}{\mathbf{e}}
\DeclareMathOperator{\bff}{\mathbf{f}}
\DeclareMathOperator{\bg}{\mathbf{g}}
\DeclareMathOperator{\bh}{\mathbf{h}}
\DeclareMathOperator{\bi}{\mathbf{i}}
\DeclareMathOperator{\bj}{\mathbf{j}}
\DeclareMathOperator{\bk}{\mathbf{k}}
\DeclareMathOperator{\bl}{\mathbf{l}}
\DeclareMathOperator{\bm}{\mathbf{m}}
\DeclareMathOperator{\bn}{\mathbf{n}}
\DeclareMathOperator{\bo}{\mathbf{o}}
\DeclareMathOperator{\bp}{\mathbf{p}}
\DeclareMathOperator{\bq}{\mathbf{q}}
\DeclareMathOperator{\br}{\mathbf{r}}
\DeclareMathOperator{\bs}{\mathbf{s}}
\DeclareMathOperator{\bt}{\mathbf{t}}
\DeclareMathOperator{\bu}{\mathbf{u}}
\DeclareMathOperator{\bv}{\mathbf{v}}
\DeclareMathOperator{\bw}{\mathbf{w}}
\DeclareMathOperator{\bx}{\mathbf{x}}
\DeclareMathOperator{\by}{\mathbf{y}}
\DeclareMathOperator{\bz}{\mathbf{z}}

\DeclareMathOperator{\bA}{\mathbf{A}}
\DeclareMathOperator{\bB}{\mathbf{B}}
\DeclareMathOperator{\bC}{\mathbf{C}}
\DeclareMathOperator{\bD}{\mathbf{D}}
\DeclareMathOperator{\bE}{\mathbf{E}}
\DeclareMathOperator{\bF}{\mathbf{F}}
\DeclareMathOperator{\bG}{\mathbf{G}}
\DeclareMathOperator{\bH}{\mathbf{H}}
\DeclareMathOperator{\bI}{\mathbf{I}}
\DeclareMathOperator{\bJ}{\mathbf{J}}
\DeclareMathOperator{\bK}{\mathbf{K}}
\DeclareMathOperator{\bL}{\mathbf{L}}
\DeclareMathOperator{\bM}{\mathbf{M}}
\DeclareMathOperator{\bN}{\mathbf{N}}
\DeclareMathOperator{\bO}{\mathbf{O}}
\DeclareMathOperator{\bP}{\mathbf{P}}
\DeclareMathOperator{\bQ}{\mathbf{Q}}
\DeclareMathOperator{\bR}{\mathbf{R}}
\DeclareMathOperator{\bS}{\mathbf{S}}
\DeclareMathOperator{\bT}{\mathbf{T}}
\DeclareMathOperator{\bU}{\mathbf{U}}
\DeclareMathOperator{\bV}{\mathbf{V}}
\DeclareMathOperator{\bW}{\mathbf{W}}
\DeclareMathOperator{\bX}{\mathbf{X}}
\DeclareMathOperator{\bY}{\mathbf{Y}}
\DeclareMathOperator{\bZ}{\mathbf{Z}}

\DeclareMathOperator{\balpha}{\boldsymbol{\alpha}}
\DeclareMathOperator{\bbeta}{\boldsymbol{\beta}}
\DeclareMathOperator{\bdelta}{\boldsymbol{\delta}}
\DeclareMathOperator{\bepsilon}{\boldsymbol{\epsilon}}
\DeclareMathOperator{\bchi}{\boldsymbol{\chi}}
\DeclareMathOperator{\beeta}{\boldsymbol{\eta}}
\DeclareMathOperator{\bgamma}{\boldsymbol{\gamma}}
\DeclareMathOperator{\biota}{\boldsymbol{\iota}}
\DeclareMathOperator{\bkappa}{\boldsymbol{\kappa}}
\DeclareMathOperator{\blambda}{\boldsymbol{\lambda}}
\DeclareMathOperator{\bmu}{\boldsymbol{\mu}}
\DeclareMathOperator{\bnu}{\boldsymbol{\nu}}
\DeclareMathOperator{\bomega}{\boldsymbol{\omega}}
\DeclareMathOperator{\bphi}{\boldsymbol{\phi}}
\DeclareMathOperator{\bpi}{\boldsymbol{\pi}}
\DeclareMathOperator{\bpsi}{\boldsymbol{\psi}}
\DeclareMathOperator{\brho}{\boldsymbol{\rho}}
\DeclareMathOperator{\bsigma}{\boldsymbol{\sigma}}
\DeclareMathOperator{\btau}{\boldsymbol{\tau}}
\DeclareMathOperator{\btheta}{\boldsymbol{\theta}}
\DeclareMathOperator{\bupsilon}{\boldsymbol{\upsilon}}
\DeclareMathOperator{\bvarepsilon}{\boldsymbol{\varepsilon}}
\DeclareMathOperator{\bvarphi}{\boldsymbol{\varphi}}
\DeclareMathOperator{\bvartheta}{\boldsymbol{\vartheta}}
\DeclareMathOperator{\bvarrho}{\boldsymbol{\varrho}}
\DeclareMathOperator{\bxi}{\boldsymbol{\xi}}
\DeclareMathOperator{\bzeta}{\boldsymbol{\zeta}}

\DeclareMathOperator{\bDelta}{\boldsymbol{\Delta}}
\DeclareMathOperator{\bGamma}{\boldsymbol{\Gamma}}
\DeclareMathOperator{\bLambda}{\boldsymbol{\Lambda}}
\DeclareMathOperator{\bOmega}{\boldsymbol{\Omega}}
\DeclareMathOperator{\bPhi}{\boldsymbol{\Phi}}
\DeclareMathOperator{\bPi}{\boldsymbol{\Pi}}
\DeclareMathOperator{\bPsi}{\boldsymbol{\Psi}}
\DeclareMathOperator{\bSigma}{\boldsymbol{\Sigma}}
\DeclareMathOperator{\bTheta}{\boldsymbol{\Theta}}
\DeclareMathOperator{\bUpsilon}{\boldsymbol{\Upsilon}}
\DeclareMathOperator{\bXi}{\boldsymbol{\Xi}}

\DeclareMathOperator{\0}{\boldsymbol{0}}
\DeclareMathOperator{\1}{\boldsymbol{1}}
\DeclareMathOperator{\2}{\boldsymbol{2}}
\DeclareMathOperator{\3}{\boldsymbol{3}}
\DeclareMathOperator{\4}{\boldsymbol{4}}
\DeclareMathOperator{\5}{\boldsymbol{5}}
\DeclareMathOperator{\6}{\boldsymbol{6}}
\DeclareMathOperator{\7}{\boldsymbol{7}}
\DeclareMathOperator{\8}{\boldsymbol{8}}
\DeclareMathOperator{\9}{\boldsymbol{9}}

% # PLAIN TYPEFACE MATHEMATICS

\DeclareMathOperator{\ra}{\mathrm{a}}
\DeclareMathOperator{\rb}{\mathrm{b}}
\DeclareMathOperator{\rc}{\mathrm{c}}
\DeclareMathOperator{\rd}{\mathrm{d}}
\DeclareMathOperator{\re}{\mathrm{e}}
\DeclareMathOperator{\rf}{\mathrm{f}}
\DeclareMathOperator{\rg}{\mathrm{g}}
\DeclareMathOperator{\rh}{\mathrm{h}}
\DeclareMathOperator{\ri}{\mathrm{i}}
\DeclareMathOperator{\rj}{\mathrm{j}}
\DeclareMathOperator{\rk}{\mathrm{k}}
\DeclareMathOperator{\rl}{\mathrm{l}}
\DeclareMathOperator{\rmm}{\mathrm{m}}
\DeclareMathOperator{\rn}{\mathrm{n}}
\DeclareMathOperator{\ro}{\mathrm{o}}
\DeclareMathOperator{\rp}{\mathrm{p}}
\DeclareMathOperator{\rqq}{\mathrm{q}}
\DeclareMathOperator{\rr}{\mathrm{r}}
\DeclareMathOperator{\rs}{\mathrm{s}}
\DeclareMathOperator{\rt}{\mathrm{t}}
\DeclareMathOperator{\ru}{\mathrm{u}}
\DeclareMathOperator{\rv}{\mathrm{v}}
\DeclareMathOperator{\rw}{\mathrm{w}}
\DeclareMathOperator{\rx}{\mathrm{x}}
\DeclareMathOperator{\ry}{\mathrm{y}}
\DeclareMathOperator{\rz}{\mathrm{z}}


% # REFERENCE - MUST COME AFTER MATH ENVS
\usepackage{cleveref}

\crefname{equation}{Eq.}{Eqs.}
\creflabelformat{equation}{#2\textup{#1}#3}
\crefname{lem}{lemma}{lemmas}
\crefname{thm}{theorem}{theorems}
\crefname{prop}{proposition}{propositions}
\crefname{cor}{corollary}{corollaries}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{White},   
    commentstyle=\color{Green},
    keywordstyle=\color{RedOrange},
    stringstyle=\color{Green},
    emphstyle=\color{RoyalPurple},
    basicstyle=\ttfamily\scriptsize,
    numberstyle=\tiny\color{Gray},
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=6pt,  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    xleftmargin=12pt,
}
\lstset{style=mystyle}
